Active Neural Mapping

We address the problem of active mapping with a continually-learned neural scene representation, namely Active Neural Mapping. The key lies in actively finding the target space to be explored with efficient agent movement, thus minimizing the map uncertainty on-the-fly within a previously unseen environment. In this paper, we examine the weight space of the continually-learned neural field, and show empirically that the neural variability, the prediction robustness against random weight perturbation, can be directly utilized to measure the instant uncertainty of the neural map. Together with the continuous geometric information inherited in the neural map, the agent can be guided to find a traversable path to gradually gain knowledge of the environment. We present for the first time an active mapping system with a coordinate-based implicit neural representation for online scene reconstruction. Experiments in the visually-realistic Gibson and Matterport3D environment demonstrate the efficacy of the proposed method.

==> srcs/representation.tex <==
\section{Preliminaries}
\label{sec:pre}

\subsection{Modern INR Architectures}
We here revisit four modern INR achitectures that fall into two kinds: the compositional depth networks of \emph{SIREN}~\cite{Sitzmann2020nips} and \emph{FourFeat}~\cite{Tancik2020nips}, and the multiplicative filter networks~\cite{Fathony2021iclr} of \emph{GaborNet} and \emph{FourierNet}. As noted by~\cite{Fathony2021iclr} and~\cite{Yuce2022cvpr}, these INRs share a similar expressive power to represent functions as a linear combination of certain harmonics $\boldsymbol{y}=\sum \bar{a}_j \sin(\bar{\boldsymbol{\omega}}_j\boldsymbol{x}+\bar{\boldsymbol{\phi}}_j)$, of which the amplitude, frequency, and phase directly depend on learned network parameters and pre-defined hyperparameters.

Denote $\boldsymbol{z}^{(l)}$ as post-activation units at each hidden layer, $\boldsymbol{W}$ and $\boldsymbol{b}$ the weights and biases of the trained network, the output $\boldsymbol{y}$ through a forward pass can be generally categorized into three stages: the input mapping stage, the spectral support expansion stage, and the final linear combination stage, which are defined as follows:
\begin{equation}
	\begin{aligned}
		\boldsymbol{z}^{(0)} & =  \gamma(\boldsymbol{x})\\ 
		\boldsymbol{z}^{(l)}  & = \rho^{(l)}(\boldsymbol{W}^{(l)}\boldsymbol{z}^{(l-1)}+\boldsymbol{b}^{(l)}), \ l=1,\cdots, L-1\\ 
		\boldsymbol{y}          & =  \boldsymbol{W}^{(L)}\boldsymbol{z}^{(L-1)}+\boldsymbol{b}^{(L)}. 
		\label{eq:INRs}
	\end{aligned}
\end{equation}

\noindent\textbf{Input mapping.} As stated in~\cite{Tancik2020nips, Yuce2022cvpr}, the input mapping $ \gamma(\boldsymbol{x})$ serves as a frequency basis instantiation, and the band limits of the frequency basis are determined by certain parameters. Following~\cite{Yuce2022cvpr}, the input mapping of \emph{SIREN} can be viewed as the first-layer post-activation $\gamma(\boldsymbol{x})=\sin(\omega_0(\boldsymbol{W}^{(0)}\boldsymbol{x}+\boldsymbol{b}^{(0)}))$,\footnote{As the first-layer post-activation serves as the input mapping, the layer $l$ starts with $2$ during harmonic expansion for SIREN.} where the range of basis frequencies are scaled by the hyperparameter $\omega_0$ and controlled by the learned weights $\boldsymbol{W}^{(0)}$. For \emph{FourFeat}, the inputs are mapped to a Gaussian Fourier feature as $\gamma(\boldsymbol{x}) = \sin(2\pi\boldsymbol{B}\boldsymbol{x}+\boldsymbol{\psi})$, where the frequency basis $\boldsymbol{B}$ are random samples from a zero-mean Gaussian distribution $\mathcal{N}(0,\sigma^2)$, and the phases $\boldsymbol{\psi}$ alternate between $0$ and $\pi/2$. The range of bais frequencies are determined by $\sigma$. 
On the other hand, the multiplicative networks~\cite{Fathony2021iclr} utilize a Gabor filter $\gamma(\boldsymbol{x})=\exp(-(\sfrac{\boldsymbol{\lambda}^{(0)}}{2})\cdot(\boldsymbol{x}-\boldsymbol{\mu}^{(0)})^2)\cdot \sin(\boldsymbol{\Omega}^{(0)}\boldsymbol{x}+\boldsymbol{\phi}^{(0)})$ and a Fourier filter $\gamma(\boldsymbol{x})=\sin(\boldsymbol{\Omega}^{(0)}\boldsymbol{x}+\boldsymbol{\phi}^{(0)})$ as the mapping functions of \emph{GaborNet} and \emph{FourierNet}. The bandwidth of basis frequencies are determined by the learned filter parameters, $\{\boldsymbol{\lambda}^{(0)}, \boldsymbol{\mu}^{(0)}, \boldsymbol{\Omega}^{(0)}, \boldsymbol{\phi}^{(0)}\}$ and $\{\boldsymbol{\Omega}^{(0)}, \boldsymbol{\phi}^{(0)}\}$ respectively.

\noindent\textbf{Spectral support expansion.} The input mapping stage defines the spectral support basis in $\boldsymbol{z}^{(0)}$: the set of frequencies that can be expressed in this stage. Afterwards, the spectral supports are extended, allowing the network to represent signals with spectrum other than the support basis. This is achieved by the function $\rho(\cdot)$ recurrently, where higher-frequency sinusoids are supported given deeper layers. For compositional depth networks of \emph{SIREN} and \emph{FourFeat}, non-linear activations ($\sin$ and ReLU non-linearities respectively) serve to expand the frequency basis into higher-frequency harmonics. This is proven by~\cite{Yuce2022cvpr} that a polynomial activation function $\rho(\boldsymbol{v}) = \sum_{k=0}^{K}a_k\boldsymbol{v}^k$, a general approximation of common non-linear activations such as $\sin$ and ReLU, transforms a single-frequency signal $e^{j\omega\boldsymbol{v}}$ into a linear combination of certain harmonics of the input frequency as $\sum_{k=0}^{K}a_k e^{j\omega k \boldsymbol{v}}$. The compositional structure of the network expands the frequency basis in $\boldsymbol{z}^{(0)} $ to the final hidden layer units $\boldsymbol{z}^{(L-1)}$ recurrently. On the other hand, the multiplicative filter networks of \emph{GaborNet} and \emph{FourierNet} employ a Hadamard product between the linear layer outputs and the filtered inputs as $\rho^{(l)}(\boldsymbol{W}^{(l)}\boldsymbol{z}^{(l-1)}+\boldsymbol{b}^{(l)})=g^{(l)}(\boldsymbol{x})\circ(\boldsymbol{W}^{(l)}\boldsymbol{z}^{(l-1)}+\boldsymbol{b}^{(l)})$, where $g^{(l)}(\boldsymbol{x})$ is the aforementioned Gabor filter or Fourier filter. Since the Hadamard product of sinusoids results in summed frequencies~\cite{Lindell2022cvpr}, the recurrent multiplication allows the network to gradually increase its bandwidth as it goes deeper. It should be noted that instead of directly learning the coefficients of the Fourier series, this recurent nature guarantees a low-rank property for both compositional depth networks and multiplicative filter networks, as proved by~\cite{Fathony2021iclr} and~\cite{Yuce2022cvpr}.

\noindent\textbf{Final linear combination.} The final output of the network is simply a linear combination of the last hidden units. That is, with varying spectral supports, each unit is weighted by the parameters of the last layer to best fit the target spectrum.

\begin{equation}
	\label{eq:mapping}
	\hat{f}(\bm{x})=\sum_{n^t}(\mathbf{K}^{-1}\bm{y})_i k(\bm{x}_i, \bm{x}).
\end{equation}



